Uncovering the ultimate planet impostor. An eclipsing brown dwarf in a hierarchical triple with two evolved stars

Exoplanet searches through space-based photometric time series have shown to be very efficient in recent years. However, follow-up efforts on the detected planet candidates have been demonstrated to be critical to uncover the true nature of the transiting objects. In this paper we show a detailed analysis of one of those false positives hidden as planetary signals. In this case, the candidate KOI-3886.01 showed clear evidence of a planetary nature from various techniques. Indeed, the properties of the fake planet set it among the most interesting and promising for the study of planetary evolution as the star leaves the main sequence. To unveil the true nature of this system, we present a complete set of observational techniques including high-spatial resolution imaging, high-precision photometric time series (showing eclipses, phase curve variations and asteroseismology signals), high-resolution spectroscopy and derived radial velocities, to unveil the true nature of this planet candidate. We find that KOI-3886.01 is an interesting false positive case: a hierarchical triple system composed by a $\sim$K2III giant star (KOI-3886A) accompanied by a close-in eclipsing binary formed by a subgiant $\sim$G4IV star (KOI-3886B) and a brown dwarf (KOI-3886C). In particular, KOI-3886C is one of the most irradiated brown dwarfs known to date, showing the largest radius in this substellar regime. It is also the first eclipsing brown dwarf known around an evolved star. In this paper we highlight the relevance of complete sets of follow-up observations to extrasolar planets detected by the transit technique using large-pixel photometers such as Kepler and TESS, and in the future, PLATO. In particular, multi-color high-spatial resolution imaging was the first hint toward ruling out the planet scenario in this system.

==> Table_BasicProp.tex <==
\begin{table}[]
%\centering
\setlength{\extrarowheight}{3pt}
\caption{\label{tab:basic} General properties of the KOI-3886 system.}
\begin{tabular}{lll}
 
 \hline 
Parameter & Value & Ref.$^{\dagger}$ \\ 
\hline 
IDs & KOI-3886, HD\,190655, \\
        &  KIC\,8848288, TIC\,185060864 \\
Gaia EDR3 ID & 2082133182277361152  & [1] \\
RA, DEC & 20:04:11.33, +45:05:15.30  &  [1]\\ 
Parallax (mas) & $2.14 \pm 0.30 $    & [1]\\
$\mu_{\alpha}$ (mas/yr) & $-8.41\pm 0.37$  & [1]\\
$\mu_{\delta}$ (mas/yr) & $-3.18\pm 0.37$  & [1]\\
RV (km/s) & $-24.00 \pm 0.64$  &  [1] \\ 
G (mag) & 10.1  &  [1]\\
$B_p-R_p$ (mag) & 1.28  &  [1]\\
m$_V$ (mag) & $10.306 \pm 0.050$ &  [2]\\
Ks (mag) & $7.475\pm0.023$ & [3] \\
U (km/s) & -3.955 & [4]\\
V (km/s) & -23.478 & [4] \\
W (km/s) & -3.026 & [4]\\
Gal. population & Thin disk & [4] \\

 \hline

\end{tabular}
\tablebib{
[1] Gaia Collaboration et al. (2016); %\citet{gaia}; 
[2] Bessell et al. (1998); %\citet{bessell98};  
[3] Cohen et al. (2003); 
[4] This work.}
\end{table}

==> Table_LC_RV_modeling.tex <==
\begin{table*}
\setlength{\extrarowheight}{3pt}
\caption{Derived stellar parameters from components B and C of the KOI-3886 hierarchical triple system through the joint (radial velocity, eclipse, and phase modulations) analysis presented in Sect.~\ref{sec:joint}.}
\label{tab:joint}
\begin{tabular}{lll}
\hline\hline
Parameter & Priors & Posteriors \\
\hline
\textit{Orbital parameters} & & \\
\hline
Orbital period, $P_C$ [days] & $\mathcal{G}$(5.56648691,0.0001) & $5.566513^{+0.000043}_{-0.000043}$ \\
Time of mid-transit, $T_{\rm 0,C}-2400000$ [days] & $\mathcal{G}$(54966.03305,0.008) & $54966.0334^{+0.0012}_{-0.0012}$ \\
Orbital inclination, $i_{\rm C}$ [deg.] & $\mathcal{U}$(70.0,90.0) & $82.50^{+0.58}_{-0.53}$ \\
Orbit semi-major axis, $a_{C}$ [AU] & (derived) & $0.0720^{+0.0013}_{-0.0013}$ \\
Relative orbital separation, $a_{C}/R_{\star}$ & (derived) & $4.287^{+0.093}_{-0.085}$ \\
Incident Flux, $F_{\rm inc,C}$ [$F_{{\rm inc},\oplus}$] & (derived) & $126.6^{+4.0}_{-2.6}$ \\

\hline
\textit{Star B} & & \\
\hline
Stellar mass, $M_{B}$ [$M_{\odot}$] & $\mathcal{T}$(1.6,0.1,1.4,1.8) & $1.608^{+0.087}_{-0.088}$ \\
Stellar radius, $R_{B}$ [$R_{\odot}$] & $\mathcal{T}$(3.5,0.3,2.5,4.5) & $3.61^{+0.11}_{-0.12}$ \\
Limb darkening coefficient, $u_1$ & $\mathcal{G}$(0.592,0.02) & $0.569^{+0.019}_{-0.020}$ \\
Limb darkening coefficient, $u_2$ & $\mathcal{G}$(0.141,0.02) & $0.131^{+0.020}_{-0.020}$ \\

\hline
\textit{Star C} & & \\
\hline
Stellar mass, $M_{C}$ [$M_{\rm Jup}$] & $\mathcal{U}$(0.0,55000.0) & $66.1^{+4.1}_{-3.2}$ \\
Stellar radius, $R_{C}$ [$R_{\rm Jup}$] & $\mathcal{U}$(0.0,100.0) & $1.524^{+0.070}_{-0.072}$ \\
Eclipse depth, $\Delta_{C}$ [ppt] & (derived) & $1.880^{+0.089}_{-0.088}$ \\
Eclipse duration, $T_{\rm 14,C}$ [hours] & (derived) & $8.873^{+0.071}_{-0.070}$ \\

\hline
\textit{Instrumental parameters} & & \\
\hline
LC level & $\mathcal{U}$(-500.0,500.0) & $58.9^{+6.7}_{-5.8}$ \\
Dilution factor & $\mathcal{T}$(0.28,0.01,0.2,0.4) & $0.2765^{+0.010}_{-0.0096}$ \\
LC jitter [ppm] & $\mathcal{U}$(0.0,2000.0) & $53.0^{+1.2}_{-1.1}$ \\
$\delta_{\rm HERMES}$ [km/s] & $\mathcal{U}$(-40.0,0.0) & $-25.86^{+0.42}_{-0.41}$ \\
$\sigma_{\rm HERMES}$ [km/s] & $\mathcal{U}$(0.0,2.1) & $1.81^{+0.20}_{-0.24}$ \\
$\delta_{\rm CAFE2}$ [km/s] & $\mathcal{U}$(-35.0,-10.0) & $-23.63^{+0.18}_{-0.17}$ \\
$\sigma_{\rm CAFE2}$ [km/s] & $\mathcal{U}$(0.0,2.0) & $0.66^{+0.17}_{-0.12}$ \\

\hline

\end{tabular}
\end{table*}


==> Table_StellarParams_AB.tex <==
\begin{table}[!htb]
\caption{Parameters of stars A and B as derived in Sect.~\ref{Sect:PARAMS}.}
\label{Table:PARAMS}
\begin{tabular}{ccccc}
  \hline\hline
  \noalign{\smallskip}
Star  & $T_{\rm eff}$ (K) &  $M_*/M_\odot$ & $R_*/R_\odot$ & $L_*/L_\odot$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
 A    & 4600$\pm$100  & 1.75$\pm$0.10 & 10.40$\pm$0.10 & 43.3$\pm$9.5 \\ 
 B    & 5600$\pm$100  & 1.61$\pm$0.05 &  3.61$\pm$0.09 & 11.5$\pm$1.0 \\
\noalign{\smallskip}\hline
\end{tabular}
\end{table}

==> Table_photometry.tex <==
\begin{table*}[!htb]
\caption{Photometry of KOI-3886.}
\label{Table:PHOT}
\setlength{\tabcolsep}{10pt}
\begin{tabular}{rrcll}
  \hline\hline
  \noalign{\smallskip}
 \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{Magnitude}   &   Flux  & Band & Source \\
 \multicolumn{1}{c}{(\AA)}     &                       & (erg cm$^{-2}$ s$^{-1}$ \AA$^{-1}$) & & \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
 2315.7 & 17.169$\pm$0.013  & 2.754(-15)$\pm$3.297(-17) & GALEX NUV$^\dagger$ & \cite{Beitia16}\\ 
 3660   & 12.016$\pm$0.022  & 6.520(-14)$\pm$1.321(-15) & Johnson $U$ & \cite{Bessell98}    \\
 4220   & 11.447$\pm$0.091  & 1.794(-13)$\pm$1.505(-14) & Tycho $B$  & \cite{Mann15}     \\
 4380   & 11.198$\pm$0.027  & 2.097(-13)$\pm$5.214(-15) & Johnson $B$ & \cite{Bessell98}     \\
 4770   & 10.706$\pm$0.020  & 2.497(-13)$\pm$4.599(-15) & Sloan $g'$ & \cite{Fukugita96,York00}   \\
 5350   & 10.352$\pm$0.054  & 2.914(-13)$\pm$1.450(-14) & Tycho $V$ & \cite{Mann15}      \\
 5450   & 10.306$\pm$0.050  & 2.739(-13)$\pm$1.262(-14) & Johnson $V$ & \cite{Bessell98}     \\
 6230   &  9.782$\pm$0.020  & 3.428(-13)$\pm$6.315(-15) & Sloan $r'$ & \cite{Fukugita96,York00} \\
 7620   &  9.465$\pm$0.020  & 3.069(-13)$\pm$5.653(-15) & Sloan $i'$ & \cite{Fukugita96,York00}   \\
 9130   &  9.288$\pm$0.020  & 2.516(-13)$\pm$4.636(-15) & Sloan $z'$ & \cite{Fukugita96,York00}  \\
12350   &  8.159$\pm$0.020  & 1.705(-13)$\pm$3.141(-15) & 2MASS $J$ & \cite{Cohen03}     \\
16620   &  7.638$\pm$0.020  & 9.978(-14)$\pm$1.838(-15) & 2MASS $H$ & \cite{Cohen03}       \\
21590   &  7.475$\pm$0.023  & 4.383(-14)$\pm$9.284(-16) & 2MASS $K_{\rm s}$ & \cite{Cohen03} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\multicolumn{4}{l}{$\dagger$ GALEX NUV magnitude is available from Vizier catalogue:}\\
\multicolumn{4}{l}{\url{https://vizier.u-strasbg.fr/viz-bin/VizieR?-source=J/ApJ/813/100}}
\end{tabular}
\end{table*}



==> Table_starA.tex <==
\begin{table}[]
%\centering
\setlength{\extrarowheight}{3pt}
\caption{\label{tab:starA} Spectroscopic (Sect.~\ref{sec:spec_analysis}) and asteroseismology (Sect.~\ref{sec:asteroseismology}) parameters of \kA{}.}
\begin{tabular}{lc}
 
 \hline 
Parameter & \kA{}  \\ 
\hline 
\textit{Spectroscopy} \\
\hline
Effective temperature, $T_{\rm eff,A}$ & $4720\pm120$~K\\
Surface gravity, $\log{g}_{\rm A}^{\rm spec}$ & $2.54\pm0.24$ \\
Turbulent velocity, $v_{\rm turb}$ & $1.172\pm0.095$~km/s \\
Metallicity, [Fe/H] & $0.143 \pm0.065$ \\
 \hline
\textit{Asteroseismology} \\
\hline
Stellar mass, $M_{\rm \star,A}$ & $1.69^{+0.14}_{-0.10}~M_{\odot}$ \\
Stellar radius, $R_{\rm \star,A}$ & $11.13^{+0.32}_{-0.26}~R_{\odot}$ \\
Stellar luminosity, $L_{\rm \star,A}$ & $55.1^{+5.2}_{-2.4}~L_{\odot}$ \\
Surface gravity, $\log{g}_{\rm \star,A}^{\rm ast}$ &$2.577^{+0.011}_{-0.009}$ \\
Stellar age & $2.05^{+0.56}_{-0.28}$~Gyr \\
 \hline
 
 \end{tabular}

\end{table}
